SALVe: Semantic Alignment Verification for Floorplan Reconstruction from Sparse Panoramas

We propose a new system for automatic 2D floorplan reconstruction that is enabled by SALVe, our novel pairwise learned alignment verifier. The inputs to our system are sparsely located 360$^\circ$ panoramas, whose semantic features (windows, doors, and openings) are inferred and used to hypothesize pairwise room adjacency or overlap. SALVe initializes a pose graph, which is subsequently optimized using GTSAM. Once the room poses are computed, room layouts are inferred using HorizonNet, and the floorplan is constructed by stitching the most confident layout boundaries. We validate our system qualitatively and quantitatively as well as through ablation studies, showing that it outperforms state-of-the-art SfM systems in completeness by over 200%, without sacrificing accuracy. Our results point to the significance of our work: poses of 81% of panoramas are localized in the first 2 connected components (CCs), and 89% in the first 3 CCs. Code and models are publicly available at https://github.com/zillow/salve.

==> latex/tex/hnet_eval_table.tex <==






% \begin{table}[]
%     \centering
%     \begin{adjustbox}{max width=\columnwidth}
% 	\begingroup
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%         \textsc{Model Name} & \textsc{dense room shape}  & \textsc{Door F1} & \textsc{Window F1} & \textsc{Opening F1} \\
%         %& \textsc{2d IoU} & \textsc{@ 50\% IoU} & \textsc{@ 50\% IoU} & \textsc{@ 50\% IoU} \\
%         & \textsc{2d IoU} & \textsc{@ 70\% IoU} & \textsc{@ 70\% IoU} & \textsc{@ 70\% IoU} \\
%     \midrule
%       % \textsc{HorizonNet} & 0.846 & 0.898 & 0.921 & 0.715 \\ % @ 50% IoU
%       \textsc{HorizonNet} & 0.846 & 0.890 &  0.912 & 0.669 \\ % @ 70% IoU
%     \bottomrule
%     \end{tabular}
%     \endgroup
%     \end{adjustbox}
%     \caption{Layout estimation and object detection accuracy of our HorizonNet model on the ZinD test set. A true positive for F1 score is defined here as 70\% 1d IoU overlap (we also provide an evaluation at 50\% and 90\% 1d IoU in the supplementary).  %Could also measure depth error to the shape (for true positives).
%     }
%     \label{tab:hnet-accuracy}
% \end{table}


